Beyond the Next Token: Towards Prompt-Robust Zero-Shot Classification via Efficient Multi-Token Prediction

Zero-shot text classification typically relies on prompt engineering, but the inherent prompt brittleness of large language models undermines its reliability. Minor changes in prompt can cause significant discrepancies in model performance. We attribute this prompt brittleness largely to the narrow focus on nexttoken probabilities in existing methods. To address this, we propose Placeholding Parallel Prediction (P3), a novel approach that predicts token probabilities across multiple positions and simulates comprehensive sampling of generation paths in a single run of a language model. Experiments show improved accuracy and up to 98% reduction in the standard deviation across prompts, boosting robustness. Even without a prompt, P3 maintains comparable performance, reducing the need for prompt engineering.

==> figs_tables/_bak/greedyoutput.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{cr|c}
\toprule
Input                                      &                           & \multicolumn{1}{c}{Output}                                                                                                                                                                          \\ \hline
\multirow{2}{*}{My ACL paper is accepted.} & \multirow{2}{*}{It is \_} & \multirow{2}{*}{\textcolor{blue}{a very} \textcolor{red}{good} paper.}                                                                                        \\
                                           &                           &                                                                                                                                                                                                     \\
\multirow{2}{*}{My legs are broken.}       & \multirow{2}{*}{I am \_}  & \multirow{2}{*}{\textcolor{blue}{in a lot of} \textcolor{red}{pain}.}                                                                                         \\
                                           &                           &                                                                                                                                                                                                     \\
I had my first job this year.              & It is \_                  & \begin{tabular}[c]{@{}c@{}}\textcolor{blue}{a part-time job at a local restaurant.}\\ \textcolor{blue}{I am a waitress. I} \textcolor{red}{like} my job very much.\end{tabular} \\ 
\bottomrule
\end{tabular}

\caption{
Greedy output examples from LLaMa2-13B. \textcolor{blue}{Blue} text indicates non-discriminative expressions and \textcolor{red}{red} text indicates discriminative words for target categories \{positive, negative\}.
}

\label{tab:greedyOutputs}
\end{table*}

==> figs_tables/usedsamples.tex <==
\begin{table}[!h]
    \centering
    \resizebox{0.85\linewidth}{!}{
    \begin{tabular}{l|cc}
    \toprule
       \textbf{ Dataset }& \textbf{ \(\tilde{\phi}(l_t)\) } & \textbf{Samples Used} \\ \midrule
        IMDb & \(0.75 \cdot (l\_t + 10)\) & 22877 / 25000 \\ %\hline
        AGnews & \(1.7 \cdot (l\_t + 10)\) & 7599 / 7600 \\ %\hline
        CaReR & \(1.4 \cdot (l\_t + 10)\) & 2000 / 2000 \\ %\hline
        DBpedia & \(1.9 \cdot (l\_t + 10)\) & 69958 / 70000 \\ %\hline
        ISEAR & \(0.15 \cdot (l\_t + 10)\) & 7666 / 7666 \\ %\hline
        SST-2 & \(0.1 \cdot (l\_t + 10)\) & 1821 / 1821 \\ %\hline
        Yahoo & \(2.1 \cdot (l\_t + 10)\) & 50547 / 60000 \\ \bottomrule
    \end{tabular}}


    \caption{
    The linear approximation of positional indexes of well-performing tokens \(\tilde{\phi}(l_t)\) for each dataset, with the slope \(k\) as a hyperparameter and intercept \(b=-10\).
    Due to experimental constraints, we could only compare the next-token and the first 512 subsequent tokens. 
    When the input data length caused \(\tilde{\phi}(l_t)\) to fall outside the [0,512] range, we had to exclude these excessively long data samples to ensure a fair comparison.
    }



    \label{tab:phi}
\end{table}
